Iterative Domain-Repaired Back-Translation

In this paper, we focus on the domain-specific translation with low resources, where in-domain parallel corpora are scarce or nonexistent. One common and effective strategy for this case is exploiting in-domain monolingual data with the back-translation method. However, the synthetic parallel data is very noisy because they are generated by imperfect out-of-domain systems, resulting in the poor performance of domain adaptation. To address this issue, we propose a novel iterative domain-repaired back-translation framework, which introduces the Domain-Repair (DR) model to refine translations in synthetic bilingual data. To this end, we construct corresponding data for the DR model training by round-trip translating the monolingual sentences, and then design the unified training framework to optimize paired DR and NMT models jointly. Experiments on adapting NMT models between specific domains and from the general domain to specific domains demonstrate the effectiveness of our proposed approach, achieving 15.79 and 4.47 BLEU improvements on average over unadapted models and back-translation.

==> tables/iter-ape-acc.tex <==
% Table generated by Excel2LaTeX from sheet 'Iterative join training'
\begin{table}[t]
\footnotesize
    \centering
      \begin{tabular}{c||ccc}
      \toprule
      No. Iter. & $\bigtriangleup$ iter-BT & $\bigtriangleup$ iter-DAPE & Diff. \\
      \hline
      \hline
      0     & 0.00  & 0.00  & 0.00  \\
      1     & 8.22  & 10.46  & 2.24  \\
      2     & 1.44  & 5.26  & 6.06  \\
      3     & 4.74  & 3.00  & 4.32  \\
      4     & 0.63  & 1.83  & 5.53  \\
      \bottomrule
      \end{tabular}%
      \caption{BLEU scores(\%) changes. $\bigtriangleup$ iter-BT and $\bigtriangleup$ iter-DAPE represent the BLEU increment of iter-BT and iter-DAPE compared with the previous iteration, respectively. Diff. represents the diffrence between iter-DAPE and iter-BT in the same iteration.}
    \label{tab:iter-ape-acc}%
  \end{table}%  

==> tables/main-results-spec2spec.tex <==
% Table generated by Excel2LaTeX from sheet '领域见适应表格'
\begin{table*}[t]
  \centering
    \begin{tabular}{||l||c|c|c|c|c|c||}
    \multicolumn{1}{||c||}{\multirow{2}[3]{*}{\textbf{Method}}} & \multicolumn{2}{c|}{\textbf{IT}} & \multicolumn{2}{c|}{\textbf{LAW}} & \multicolumn{2}{c||}{\textbf{MED}} \\
\cmidrule{2-7}          & \textbf{LAW} & \textbf{MED} & \textbf{IT} & \textbf{MED} & \textbf{IT} & \textbf{LAW} \\
    \midrule
    \midrule
    \newcite{Dou2019UnsupervisedDA} & 11.67  & 21.30  & 15.41  & 26.96  & 13.03  & 14.28  \\
    \newcite{Hu2019DomainAO} & 8.75  & 19.49  & 11.65  & 26.98  & 10.99  & 11.32  \\
    \midrule
    Baseline & 4.71  & 8.75  & 5.82  & 14.02  & 5.30  & 7.52  \\
    Copy  & 5.11  & 11.15  & 7.57  & 19.23  & 5.89  & 6.01  \\
    BT    & 12.93  & 20.66  & 18.96  & 30.20  & 15.62  & 16.39  \\
    DALI  & 8.42  & 18.04  & 10.64  & 24.24  & 10.45  & 10.23  \\
    DALI-BT & 13.26  & 22.13  & 18.05  & 33.50  & 16.96  & 16.40  \\
    iter1 BT & 14.31  & 25.05  & 25.35  & 33.86  & 20.48  & 23.14  \\
    \midrule
    APE-BT & 15.17  & 24.87  & 23.75  & 35.41  & 20.18  & 20.15  \\
    iter1 APE-BT & \textbf{20.54 } & \textbf{33.58 } & \textbf{27.79 } & \textbf{41.47 } & \textbf{25.52 } & \textbf{26.28 } \\
    \end{tabular}%
    \caption{Add caption}
  \label{tab:main-results-spec2spec}%
\end{table*}%

